Semifinite von Neumann algebras in gauge theory and gravity

von Neumann algebras have been playing an increasingly important role in the context of gauge theories and gravity. The crossed product presents a natural method for implementing constraints through the commutation theorem, rendering it a useful tool for constructing gauge invariant algebras. The crossed product of a Type III algebra with its modular automorphism group is semifinite, which means that the crossed product regulates divergences in local quantum field theories. In this letter, we find a sufficient condition for the semifiniteness of the crossed product of a type III algebra with any locally compact group containing the modular automorphism group. Our condition surprisingly implies the centrality of the modular flow in the symmetry group, and we provide evidence for the necessity of this condition. Under these conditions, we construct an associated trace which computes physical expectation values. We comment on the importance of this result and and its implications for subregion physics in gauge theory and gravity.

==> AlgMacros.tex <==
% last update: RGL 2022-12-15
% character macros for Lie algebroids

\usepackage{mathrsfs,mathtools}
\renewcommand\mathbb[1]{\mathbbm{#1}}
\newcommand\mathbbb[1]{\boldsymbol{\mathbb{#1}}}

% general macros
\newcommand{\Lagr}{\mathfrak{L}} % Lagrangian d-form
\newcommand{\td}{{\rm d}}
\newcommand{\ts}{{\rm s}}

% Lie algebroid macros
% spaces M,G; bundles P,L,TM,A
\newcommand{\injo}{j}
\newcommand{\hatd}{\hat{d}}
\newcommand{\hatLie}[1]{\hat{\cal L}_{#1}}
\newcommand{\hatcon}[1]{\hat{i}_{#1}}

\newcommand{\mX}{\un{\mathfrak{X}}}
\newcommand{\mY}{\un{\mathfrak{Y}}}
\newcommand{\mZ}{\un{\mathfrak{Z}}}
\newcommand{\mD}{\mathfrak{D}}
\newcommand{\mg}{\mathfrak{g}}
\newcommand{\mh}{\mathfrak{h}}

\newcommand{\Aconn}[1]{\phi_{#1}}
\newcommand{\AconnX}[2]{\Aconn{#1}(#2)}

% configuration algebroid macros
\newcommand{\morphalg}{\mathbbb{G}}
\newcommand{\pbalg}{\mathbbb{P}}
\newcommand{\Tpbalg}{\text{T}\pbalg}
\newcommand{\spalg}{\mathbbb{M}}
\newcommand{\Tspalg}{\text{T}\spalg}
\newcommand{\fldspalg}{\mathbbb{F}}
\newcommand{\algalg}{\mathbbb{A}}
\newcommand{\ellalg}{\mathbbb{L}}
\newcommand{\algassoc}{{\mathbbb{E}}}

\newcommand{\alghatd}{\hat{\delta}}
\newcommand{\alghatdTM}{\delta}
\newcommand{\alghatdL}{\sigma}
\newcommand{\algvec}[1]{\mathbb{V}_{#1}}
\newcommand{\algLie}[1]{\hat{\text{L}}_{#1}}
\newcommand{\algcon}[1]{\hat{\text{I}}_{{#1}}}
\newcommand{\algchg}[1]{\text{H}_{#1}}
\newcommand{\algchgdens}[1]{\text{Q}_{#1}}
\newcommand{\algcurrdens}[1]{\text{J}_{#1}}
\newcommand{\algflux}[1]{{\cal F}_{#1}}
\newcommand{\algAnom}[1]{\Delta_{#1}}

\newcommand{\algsec}[1]{\un{\bm{\mathfrak{#1}}}}
\newcommand{\algmX}{\algsec{X}}
\newcommand{\algmY}{\algsec{Y}}
\newcommand{\algmZ}{\algsec{Z}}
\newcommand{\alginjo}{\mathbbb{j}}
\newcommand{\algrho}{\mathbbb{r}}
\newcommand{\algsigma}{\mathbbb{s}}
\newcommand{\alggauge}{\mathbbb{b}}
\newcommand{\algomega}{\mathbbb{w}}

\newcommand{\coframeVb}[1]{\bm{t}^{#1}}
\newcommand{\frameHb}[1]{\un{\bm{t}}_{#1}}
\newcommand{\MCb}{\bm{\varpi}}

\newcommand{\bbmu}{\ellsec{\mu}}
\newcommand{\bbnu}{\ellsec{\nu}}

% Hamiltonian algebroid macros
\newcommand{\ellhatd}{\sigma}
\newcommand{\ellsec}[1]{\bm{#1}}

\newcommand{\Mhatd}{\delta}
\newcommand{\MLie}[1]{L_{#1}}
\newcommand{\Mcon}[1]{I_{#1}}
\newcommand{\Msec}[1]{\un{#1}}

\newcommand{\assalg}{\Omega^0(\fldspalg)}
\newcommand{\adjalg}{\mathbbb{L}}
\newcommand{\prequpb}{\mathbbb{p}}
\newcommand{\prequalg}{\mathbbb{a}}
\newcommand{\prequver}{\mathbbb{v}}
\newcommand{\prequhor}{\mathbbb{h}}
\newcommand{\prequell}{\mathbbb{\ell}}


% specialized characters for corners
\newcommand{\dM}{\mathfrak{diff}(M)}
\newcommand{\dS}{\mathfrak{diff}(S)}

\makeatletter
\DeclareRobustCommand{\loplus}{\mathbin{\mathpalette\dog@lsemi{+}}}
\DeclareRobustCommand{\lotimes}{\mathbin{\mathpalette\dog@lsemi{\times}}}
\DeclareRobustCommand{\roplus}{\mathbin{\mathpalette\dog@rsemi{+}}}
\DeclareRobustCommand{\rotimes}{\mathbin{\mathpalette\dog@rsemi{\times}}}

\newcommand{\dog@rsemi}[2]{\dog@semi{#1}{#2}{-90,90}}
\newcommand{\dog@lsemi}[2]{\dog@semi{#1}{#2}{270,90}}
\newcommand{\dog@semi}[3]{%
  \begingroup
  \sbox\z@{$\m@th#1#2$}%
  \setlength{\unitlength}{\dimexpr\ht\z@+\dp\z@\relax}%
  \makebox[\wd\z@]{\raisebox{-\dp\z@}{%
    \begin{picture}(1,1)
    \linethickness{\variable@rule{#1}}
    \roundcap
    \put(0.5,0.5){\makebox(0,0){\raisebox{\dp\z@}{$\m@th#1#2$}}}
    \put(0.5,0.5){\arc[#3]{0.5}}
    \end{picture}%
  }}%
  \endgroup
}
\newcommand{\variable@rule}[1]{%
  \fontdimen8  
  \ifx#1\displaystyle\textfont3\else
    \ifx#1\textstyle\textfont3\else
      \ifx#1\scriptstyle\scriptfont3\else
        \scriptscriptfont3\relax
  \fi\fi\fi
}
\DeclareRobustCommand{\loplus}{\mathbin{\mathpalette\dog@lsemi{+}}}




==> LeighMacro.tex <==
% last update: RGL 2022-12-15
% special macro file for research note (see template note_template.tex)

\input{packages.tex}
\input{standard.tex}
\usepackage{mdframed,framed}

% set up sans serif fonts in text and in mathmode
\renewcommand{\familydefault}{\sfdefault}
\usepackage{sfmath}

% generic pages setups
\textwidth = 7 in
\textheight = 9.0 in
\oddsidemargin = -0.25 in
\evensidemargin = -0.25 in
\topmargin = -0.5 in
\headheight = 0.0 in
\headsep = 0.0 in
\parskip = 0.2in
\parindent = 0.2in
%
%\newcommand{\comment}[1]{}

\newcommand{\margnote}[1]{\marginpar{#1}}

\setlength\cftparskip{-1pt}
\setlength\cftbeforesecskip{5pt}
\setlength\cftaftertoctitleskip{2pt}

% Boxes
\def\mybox#1{\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{#1}}}
\def\mytbox#1#2{\noindent
	\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{{\bf #1}}}\\ 
	\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{#2}}
	}

% shaded quote box
\mdfdefinestyle{MyShadeQuoteStyle}{%
    leftmargin=15pt,
    rightmargin=15pt,
    backgroundcolor=gray!25,
    linewidth=0pt,
    skipbelow=\topskip,
    skipabove=\topskip
	}


\newenvironment{shadequote}[1][]{%
    \ignorespaces%
    \begin{mdframed}[style=MyShadeQuoteStyle,#1]%
	}{%
    \end{mdframed}%
    \ignorespacesafterend%
	}%

\newenvironment{wideshadequote}%
{\begin{snugshade}\begin{quote}}
{\hfill\end{quote}\end{snugshade}}

\definecolor{shadecolor}{rgb}{0.9,0.9,0.9}

% the title box for notes
\newlength{\leftfield}          \setlength{\leftfield}{1.5in}
\newlength{\centerfield}        \setlength{\centerfield}{3.4in}
\newlength{\rightfield}         \setlength{\rightfield}{1.9in}
								\setlength{\fboxrule}{1px}
								
\newcommand{\twodigits}[1]{\ifnum#1<10 0\fi\number#1}
	
\newcommand{\mytitlebox}[4]{
	\framebox[\textwidth]{
	\begin{minipage}[c]{\textwidth}
		\makebox[\leftfield][l]{\littlefig{Physics-logo-small.png}{3} 
		%\littlefig{PI_logo.png}{1.3}
		}\ 
		\begin{minipage}[b]{\centerfield}
			\begin{center}{\bf\large #1}\\ #2\end{center}
		\end{minipage} 
		\begin{minipage}[b]{\rightfield}
			\begin{flushright}
				#3\\ Create: #4\\ Update: \the\year--\twodigits\month--\twodigits\day 
			\end{flushright}
		\end{minipage} 
	\end{minipage}
	}
}	

\setlength{\headsep}{4 ex}
\pagestyle{myheadings}
\markright{\title\ (\author)}

%\RequirePackage{color}

% display references as hyperlinks
\newcommand{\displayref}[2]{\href[pdfnewwindow]{#1}{{\color{BrickRed}[#2]}}}

\newcounter{example}
\setcounter{example}{0}
\renewcommand{\theexample}{\arabic{section}.\arabic{example}}
\newcommand*\examplelabel[1]{\hspace\labelsep\normalfont\bfseries #1}
\newenvironment{example}[1]{\refstepcounter{example}\label{exmpl:#1}\let\makelabel\examplelabel
    \begin{mdframed}[
       frametitle={{\bf Example \theexample: #1}},
       frametitlerule=true,
       frametitlebackgroundcolor=black!20,
       frametitlebelowskip=0.5\topskip,
       outerlinewidth = 1,
       roundcorner = 5pt,
       leftmargin=20pt,
       rightmargin=20pt,
       innerleftmargin=10pt,
       innerlinewidth=1.0pt,
       innertopmargin=0.5\topskip
    ]
}{
    \end{mdframed}
}


==> packages.tex <==
% last update: RGL 2022-12-15
% standard paper packages

\usepackage{amsmath,amssymb,amsfonts,bbm,bm}
\usepackage{slashed}

\usepackage{tocloft} % well-formatted table of contents

\usepackage[nosort]{cite} % better citation format
\usepackage{graphicx,color}
\usepackage[colorlinks=true, linkcolor=blue, citecolor=blue, linktoc=all]{hyperref}

% set up color
\usepackage[usenames,dvipsnames]{xcolor}

\usepackage{tikz-cd}
\usepackage{pict2e}
\usepackage{physics}
\usepackage{comment} 
\usepackage[makeroom]{cancel}

%%%%%%%%% MARGINS %%%%%%%%%%
\setlength{\topmargin}{-0.6in}
\setlength{\textheight}{9.2in}
\setlength{\textwidth}{7in}
\setlength{\oddsidemargin}{-0.25in}
\setlength{\evensidemargin}{-0.25in}



==> standard.tex <==
% last update: RGL 2022-12-15
% common macros used in all work

% standard macros
\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\ack}[1]{[{\bf Pfft!: {#1}}]}

\newcommand{\un}[1]{\underline{#1}}
\def\pa{\partial}
\usepackage[normalem]{ulem}
\renewcommand{\uuline}[1]{\underline{\underline{#1}}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\hlt}[1]{{\color{Emerald}{\em #1}}}

% Levi-Civita characters
\newcommand{\LCGamma}{\mathring{\Gamma}}
\newcommand{\LCnabla}{\mathring{\nabla}}
\newcommand{\LCgamma}{\mathring{\gamma}}
\newcommand{\LCtnabla}{\mathring{\tilde{\nabla}}}
\newcommand{\LCW}{\mathring{W}}
\newcommand{\LCR}{\mathring{R}}






% Figure format
% usage is \myfig{filename}{w}{Caption}; where 'w' is the desired width in cm
% note: use filename root only
% -- then pdftex uses .pdf, dvips uses .eps
% a label is generated automatically
% -- use \ref{filename} to refer to figure
\newcommand{\myfig}[3]{
	\begin{figure}[h]
	\centering
	\includegraphics[width=#2cm]{figs/#1}\caption{{\scriptsize #3}}\label{fig:#1}
	\end{figure}
	}
\newcommand{\littlefig}[2]{
	\includegraphics[width=#2cm]{figs/#1}
	}


% addresses
\newcommand{\perimeter}[1]{
	\centerline{
		\begin{minipage}[c]{0.7\textwidth}
			\begin{center}~
			${}^{#1}$ Perimeter Institute for Theoretical Physics,\\
			 31 Caroline St. N., Waterloo ON, Canada, N2L 2Y5
			\end{center}
		\end{minipage}
		}
	}
\newcommand{\uiuc}[1]{
	\centerline{
		\begin{minipage}[c]{0.7\textwidth}
			\begin{center}
			${}^{#1}$ Illinois Center for Advanced Studies of the Universe \& Department of Physics,\\ 
			University of Illinois, 1110 West Green St., Urbana IL 61801, U.S.A.
			\end{center}
		\end{minipage}
		}
	}
\newcommand{\vt}[1]{
	\centerline{
		\begin{minipage}[c]{0.7\textwidth}
			\begin{center}
			${}^{#1}$ Department of Physics, Virginia Tech, Blacksburg, VA 24061, U.S.A.
			\end{center}
		\end{minipage}
		}
	}
\newcommand{\poland}[1]{
	\centerline{
		\begin{minipage}[c]{0.7\textwidth}
			\begin{center}
			${}^{#1}$ University of Wroc\l{}aw, Faculty of Physics and Astronomy, pl.\ M.\ Borna 9, 50-204 Wroc\l{}aw, Poland\\
National Centre for Nuclear Research, Pasteura 7, 02-093 Warsaw, Poland
			\end{center}
		\end{minipage}
		}
	}



